A Pain Assessment Framework based on multimodal data and Deep Machine Learning methods

From the original abstract: This thesis initially aims to study the pain assessment process from a clinical-theoretical perspective while exploring and examining existing automatic approaches. Building on this foundation, the primary objective of this Ph.D. project is to develop innovative computational methods for automatic pain assessment that achieve high performance and are applicable in real clinical settings. A primary goal is to thoroughly investigate and assess significant factors, including demographic elements that impact pain perception, as recognized in pain research, through a computational standpoint. Within the limits of the available data in this research area, our goal was to design, develop, propose, and offer automatic pain assessment pipelines for unimodal and multimodal configurations that are applicable to the specific requirements of different scenarios. The studies published in this Ph.D. thesis showcased the effectiveness of the proposed methods, achieving state-of-the-art results. Additionally, they paved the way for exploring new approaches in artificial intelligence, foundation models, and generative artificial intelligence.

==> initial/init.tex <==
\RequirePackage{fix-cm}
%\documentclass[11pt]{book}
%\documentclass[11pt,a4paper]{book}
\usepackage{subcaption}
\usepackage{minitoc} %Table_of_contents for each chapter
\usepackage{times}

\input{libtex/alias}

\usepackage{amssymb,amsfonts,amsmath}
\usepackage{epsfig}
%\usepackage{subfig}
\usepackage{url}
\usepackage{dsfont}
\usepackage[table]{xcolor}
\usepackage{multirow,tabularx}
\usepackage{paralist}
\usepackage{fancyvrb}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage[nomove]{cite}

\usepackage[flushleft]{threeparttable}
\usepackage{tablefootnote}
\usepackage{booktabs}

\usepackage{wrapfig} 

\usepackage{pifont}
\usepackage{afterpage}
\usepackage[protrusion=true,expansion=false]{microtype}
\usepackage{titlesec, blindtext}
\usepackage{lscape}
\usepackage{libtex/fancyhdr}

\usepackage{libtex/utepcsthesisReview}
\usepackage{srcltx}
\usepackage[printonlyused]{acronym}
\usepackage{setspace}
\usepackage{phaistos}
\usepackage{pifont}
%\usepackage{libertine}

\usepackage{textgreek}
\usepackage{setspace}
\usepackage[super]{nth}
\usepackage{stmaryrd}


\titleformat{\chapter}[block]
 {%\rule{1in}{1in}% (to auto-insert graphic use) \includegraphics{\chaptername-\thechapter-graphic}
 %\TitleSymbol
  \normalfont\huge\bfseries}
  {\\\chaptertitlename\ \thechapter\\}
  {0pt}
  {\Huge}
\titlespacing*{\chapter}{0pt}{0pt}{40pt}

%By default, LaTeX doesn't like to fill more than 0.7 of a text page with tables and graphics,
%nor does it like too many figures per page. This behaviour can be changed by the following:
\renewcommand\floatpagefraction{.9}
\renewcommand\topfraction{.9}
\renewcommand\bottomfraction{.9}
\renewcommand\textfraction{.1}
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}



\newcommand{\keywords}[1]{\par\addvspace\baselineskip
\noindent\keywordname\enspace\ignorespaces#1}

\long\def\comment#1{}

%%% Thesis Title %%%%
%\newcommand{\thesistitle}[0]{A Pain Assessment Framework based on multimodal data and Deep Machine Learning methods}

\newcommand{\thesistitle}[0]{A Pain Assessment Framework based on\\[0.12cm] multimodal data and Deep Machine Learning methods}




%%%%%%%%%%%%%%%%%%%%%

%%% FOR WRITING GREEK %%%
\usepackage[greek,american]{babel}
\usepackage[libtex/iso-8859-7]{inputenc}
\newcommand{\selg}[0]{\selectlanguage{greek}}
\newcommand{\selam}[0]{\selectlanguage{american}}
%%%%%%%%%%%%%%%%%%%%%%%%%




\renewcommand{\baselinestretch}{1}\small\normalsize
\textwidth=440pt
\oddsidemargin = 30pt
\evensidemargin = -16pt

\makeindex

\thispagestyle{empty} \pagestyle{empty}

%%%% FOR NEW AND INTERNAL CONTENT USE: %%%%
\newcommand{\new}[1]{{\color{red}#1}}
\newcommand{\internal}[1]{
  \footnote{
          \fbox{{\tiny InternalNote:}}
          {\tt\em
                #1
          }
      }
  }
 \newcommand{\draft}[1]{
          \noindent
          \fbox{DRAFT:}
          {\tt\bf
               #1
          }
  }


==> libtex/alias.tex <==
\long\def\comment#1{}

\newcommand{\mysection}[1]{
    \centerline{\LARGE \bf #1}
    \godown
}


\newcommand{\abstrOfeq}[0]{
     \sqsubseteq
}
\newcommand{\abstrOf}[0]{
     \sqsubset
}



% Frequently Used commands

\newcommand{\bq}{\begin{quote}}
\newcommand{\eq}{\end{quote}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bie}{\begin{itemize}\begin{enumerate}}
\newcommand{\eie}{\end{enumerate}\end{itemize}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\btbl}{\begin{tabular}}
\newcommand{\etbl}{\end{tabular}}
\newcommand{\bequ}{\begin{displaymath}}
\newcommand{\eequ}{\end{displaymath}}
\newcommand{\bequa}{\begin{eqnarray*}}
\newcommand{\eequa}{\end{eqnarray*}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\btab}{\begin{tabbing}}
\newcommand{\etab}{\end{tabbing}}
\newcommand{\cl}{\centerline}

\newcommand{\goright}{\hspace*{0.5cm}}
\newcommand{\goRight}{\goright \goright}
\newcommand{\goRIGHT}{\goRight \goRight}

\newcommand{\bul}{ $\bullet$ }
\newcommand{\goup}{ \vspace*{-0.5cm}}
\newcommand{\goUp}{ \goup \goup}
%\newcommand{\goUP}{ \vspace*{-0.5cm}}


\newcommand{\vparag}{ \vskip 5mm}
\newcommand{\godown}{ \vspace*{0.3cm}}
\newcommand{\goDown}{ \godown \godown}
\newcommand{\goDOWN}{ \goDown \goDown }

% set operator : not in
\newcommand{\noin}{\in \hspace{-0.33cm} / \hspace{0.3cm} }

%=========== MATH SYMBOLS ==============

\newcommand{\FALL}{\;\forall \;}
\newcommand{\mybox}[1]{\mbox{\letterspace #1 \letterspace }}
\newcommand{\card}[1]{
        \letterspace\mid
         #1
        \mid\letterspace
}


%=========== MDE WRITING ==============

% mpr : prints its argument in math mode
%       It can also be called from non math mode
\def\mpr#1{\ifmmode #1 \else #1 \fi}

\newcommand{\TB}        {\mpr{TB}}

%\newcommand{\R}         {\mpr{R}}
\newcommand{\RIN}       {\mpr{R^{in}}}
\newcommand{\RINALL}    {\mpr{R^{in}_{impl}}}
\newcommand{\RINB}      {\mpr{R^{in}_{sys}}}
\newcommand{\RINU}      {\mpr{R^{in}_{u}}}
\newcommand{\RINUtonos} {\mpr{R^{in'}_{u}}}
\newcommand{\RISA}      {\mpr{R^{isA}}}
\newcommand{\RISATR}    {\mpr{R^{isA}_{tr}}}
\newcommand{\RISAB}     {\mpr{R^{isA}_{sys}}}
\newcommand{\RISAU}     {\mpr{R^{isA}_{u}}}
\newcommand{\RISAUtonos}{\mpr{R^{isA'}_{u}}}
\newcommand{\RFROM}     {\mpr{R^{from}}}
\newcommand{\RTO}       {\mpr{R^{to}}}

%\newcommand{\TO}        {\mpr{O}}
\newcommand{\TOB}       {\mpr{O_{sys}}}
\newcommand{\TOU}       {\mpr{O_{u}}}
\newcommand{\PV}        {\mpr{PV}}
\newcommand{\Integer}   {\mpr{Integer}}
\newcommand{\Real}      {\mpr{Real}}
\newcommand{\String}    {\mpr{String}}
\newcommand{\Nat}       {\mpr{N}}
\newcommand{\LN}    {\mpr{L}}
\newcommand{\LF}    {\mpr{{\cal L}}}

\newcommand{\TI}        {\mpr{I}}
\newcommand{\TIU}       {\mpr{I_{u}}}
\newcommand{\TA}        {\mpr{A}}
\newcommand{\TC}        {\mpr{C}}
\newcommand{\TIC}       {\mpr{I_{c}}}
\newcommand{\TAC}       {\mpr{A_{c}}}

\newcommand{\type}      {\mpr{type}}
\newcommand{\level}     {\mpr{level}}
\newcommand{\typeb}     {\mpr{type_{sys}}}
\newcommand{\levelb}    {\mpr{level_{sys}}}

\newcommand{\SemT}      {\mpr{SemanticType}}
\newcommand{\SynT}      {\mpr{SyntacticType}}

\newcommand{\semT}      {\mpr{semType}}
\newcommand{\synT}      {\mpr{synType}}
\newcommand{\semTb}     {\mpr{semType_{sys}}}
\newcommand{\synTb}     {\mpr{synType_{sys}}}

\newcommand{\sem}       {\mpr{sem}}
\newcommand{\syn}       {\mpr{syn}}

\newcommand{\PBT}       {\mpr{PBT}}
\newcommand{\TP}        {\mpr{TP}}


\newcommand{\tellretell}{TELL/RETELL\letterspace}
\newcommand{\export}{{\em Export} \letterspace}

\newcommand{\letterspace}{\hspace*{1mm}}

\newcommand{\ison}{\;=\;}
\newcommand{\isA}{\mbox{\bf isA} \letterspace}
\newcommand{\instOf}{\mbox{\bf instOf}}

\newcommand{\Tell}{{\bf TELL Individual} \letterspace}
\newcommand{\Retell}{{\bf RETELL Individual} \letterspace}
\newcommand{\End}{{\bf end} \letterspace}
\newcommand{\inT}{{\bf in} \letterspace}
\newcommand{\scl}{{\bf S\_Class} \letterspace}
\newcommand{\tok}{{\bf Token} \letterspace}

\newcommand{\printPQI}[1]{ \mbox{\bf #1} \letterspace }

\newcommand{\sysclass}{ \printPQI{sysclass}}
\newcommand{\scn}{      \printPQI{scn}}
\newcommand{\gfv}{      \printPQI{gfv}}
\newcommand{\gtv}{      \printPQI{gtv}}
\newcommand{\glf}{      \printPQI{glf}}
\newcommand{\gilf}{     \printPQI{gilf}}
\newcommand{\gilt}{     \printPQI{gilt}}
\newcommand{\glt}{      \printPQI{glt}}
\newcommand{\glfc}{     \printPQI{glfc}}
\newcommand{\gfnc}{     \printPQI{gfnc}}
\newcommand{\gtnc}{     \printPQI{gtnc}}
\newcommand{\gasb}{     \printPQI{gasb}}
\newcommand{\gsb}{      \printPQI{gsb}}
\newcommand{\gasc}{     \printPQI{gasc}}
\newcommand{\gc}{       \printPQI{gc}}
\newcommand{\gac}{      \printPQI{gac}}
\newcommand{\gai}{      \printPQI{gai}}
\newcommand{\gi}{       \printPQI{gi}}
\newcommand{\gsc}{      \printPQI{gsc}}
\newcommand{\gSc}{      \printPQI{gSc}}
\newcommand{\gaSc}{     \printPQI{gaSc}}
\newcommand{\gSi}{      \printPQI{gSi}}
\newcommand{\attrs}{    \printPQI{attrs}}
\newcommand{\focus}     {{\em s \letterspace}}

%---------- CHAPTER 4 -------------------
\newcommand{\BPE}[1]{ \mbox{\bf #1 \letterspace} }

\newcommand{\CreateNode}        {\BPE{CreateIndividual}}
\newcommand{\DeleteNode}        {\BPE{DeleteIndividual}}
\newcommand{\CreateAttribute}   {\BPE{CreateAttribute}}
\newcommand{\DeleteAttribute}   {\BPE{DeleteAttribute}}
\newcommand{\AddInstance}       {\BPE{AddInstance}}
\newcommand{\DeleteInstance}    {\BPE{DeleteInstance}}
\newcommand{\Rename}            {\BPE{Rename}}
\newcommand{\AddSubClass}       {\BPE{AddSubClass}}
\newcommand{\DelSubClass}       {\BPE{DeleteSubClass}}
\newcommand{\makecopy}          {\BPE{MakeCopy}}

%---tmpmaybe
\newcommand{\CreateNodeSet}     {{\em CreateNodeSet}}
\newcommand{\DeleteNodeSet}     {{\em DeleteNodeSet}}
\newcommand{\CreateAttributeSet}{{\em CreateAttributeSet}}
\newcommand{\DeleteAttributeSet}{{\em DeleteAttributeSet}}
\newcommand{\AddInstanceSet}    {{\em AddInstanceSet}}
\newcommand{\DeleteInstanceSet} {{\em DeleteInstanceSet}}
\newcommand{\RenameSet}         {{\em RenameSet}}
\newcommand{\AddSubClassSet}    {{\em AddSubClassSet}}
\newcommand{\DelSubClassSet}    {{\em DelSubClassSet}}

%---------- CHAPTER 5 -------------------
\newcommand{\EFID}[1]{ \mbox{\em \scriptsize #1 } }

\newcommand{\obj}{ \letterspace
                    \mbox{\em o}\letterspace
}
\newcommand{\aobj}{ \mbox{\em a}\letterspace}
\newcommand{\bobj}{ \mbox{\em b}\letterspace}
\newcommand{\fobj}{ \mbox{\em from}\letterspace}
\newcommand{\tobj}{ \mbox{\em to}\letterspace}
\newcommand{\sobj}{ \mbox{\em s}\letterspace}
\newcommand{\cobj}{ \mbox{\em c}\letterspace}
\newcommand{\iobj}{ \mbox{\em i}\letterspace}
\newcommand{\ObjectSet}{ \mybox{\em ObjectSet}}
\newcommand{\SysClass}{ \mbox{\em SysClass}\letterspace}

\newcommand{\CREATENODE}    {\EFID{CREATE\_INDIVIDUAL}}
\newcommand{\DELETENODE}    {\EFID{DELETE\_INDIVIDUAL}}
\newcommand{\RENAMENODE}    {\EFID{RENAME\_INDIVIDUAL}}
\newcommand{\CHANGECLASSES} {\EFID{CHANGE\_CLASSES}}
\newcommand{\CHANGESUPERCLASSES}{\EFID{CHANGE\_SUPERCLASSES}}
\newcommand{\CHANGEATTRIBUTES}  {\EFID{CHANGE\_ATTRIBUTES}}
\newcommand{\nullset}   {-\hspace*{-0.1cm}-}
%%\newcommand{\emptyset}    {0\hspace*{-0.1cm}\/}
%\newcommand{\concat}   {\letterspace\#\letterspace}
\newcommand{\concat}    {\letterspace\circ\letterspace}

\newcommand{\DC}{
        \letterspace {\bf DC}\letterspace
}
\newcommand{\DO}{
        \letterspace {\bf DO}\letterspace
}
\newcommand{\RC}{${\cal R}\;$}
\newcommand{\calA}{${\cal A}\;$}
\newcommand{\calB}{${\cal B}\;$}
\newcommand{\calE}{${\cal E}\;$}

%---------- CHAPTER 6 -------------------

\newcommand{\sneg}   { \mbox{\={$\! \! \! s$}} }

\newcommand{\Users}      {Users}
\newcommand{\SystemUsers}{SystemUsers}
\newcommand{\UserTypes}  {UserTypes}

\newcommand{\Ustx}       {U_{stx}}
\newcommand{\Usem}       {U_{sem}}
\newcommand{\Tasks}      {Tasks}
\newcommand{\tsem}      {t_{sem}}
\newcommand{\apon}          {applyon}
\newcommand{\aponsem}       {applyon_{sem}}
\newcommand{\aponsemt}      {applyon^{t}_{sem}}

\newcommand{\SetIds}    {ID}
\newcommand{\tids}      {S_{id}}
\newcommand{\tidsR}     {S^{-1}_{id}}

\newcommand{\pids}      {P^{expl}_{id}}
\newcommand{\nids}      {N^{expl}_{id}}
\newcommand{\pimids}    {P^{impl}_{id}}
\newcommand{\nimids}    {N^{impl}_{id}}

\newcommand{\ti}        {S_{i}}
\newcommand{\tiR}       {S^{-1}_{i}}
\newcommand{\tj}        {S_{j}}

\newcommand{\cro}       {CrObj}
\newcommand{\delo}      {DelObj}
\newcommand{\ren}       {REN}
\newcommand{\del}       {DEL}
\newcommand{\addaf}     {AddAF}
\newcommand{\addat}     {AddAT}
\newcommand{\delaf}     {DelAF}
\newcommand{\delat}     {DelAT}
\newcommand{\addin}     {AddIn}
\newcommand{\delin}     {DelIn}
\newcommand{\addsub}    {AddSub}
\newcommand{\delsub}    {DelSub}
\newcommand{\addsup}    {AddSup}
\newcommand{\delsup}    {DelSup}
\newcommand{\addclass}  {AddClass}
\newcommand{\delclass}  {DelClass}

\newcommand{\tcro}      {S_{\cro}}
\newcommand{\tcroR}     {S^-1_{\cro}}
\newcommand{\tdelo}     {S_{\delo}}
\newcommand{\tdeloR}    {S^-1_{\delo}}
\newcommand{\tren}      {S_{\ren}}
\newcommand{\tdel}      {S_{\del}}
\newcommand{\taddaf}    {S_{\addaf}}
\newcommand{\tdelaf}    {S_{\delaf}}
\newcommand{\taddat}    {S_{\addat}}
\newcommand{\tdelat}    {S_{\delat}}
\newcommand{\taddin}    {S_{\addin}}
\newcommand{\tdelin}    {S_{\delin}}
\newcommand{\taddsub}   {S_{\addsub}}
\newcommand{\tdelsub}   {S_{\delsub}}


\newcommand{\negS}      {{\scriptsize NEG}}
\newcommand{\posS}      {{\scriptsize POS}}
\newcommand{\noneS}     {{\scriptsize NONE}}

\newcommand{\QT}    {{\cal QT}}

\newcommand{\qlevel}        {level}
\newcommand{\qlevelsub}     {levelsub}
\newcommand{\qsubs}         {subs}
\newcommand{\qgai}      {gai}
\newcommand{\qglf}      {glf}
\newcommand{\qglfgasb}  {glfgasb}

\newcommand{\Rules}     {{\cal R}}
\newcommand{\ARules}    {{\cal A}}
\newcommand{\Preds}     {{\cal PR}}
\newcommand{\PredTypes} {{\cal PRT}}
\newcommand{\PredSys}   {{\cal PR}_{sys}}
\newcommand{\PredIN}    {{\cal PR}_{in}}
\newcommand{\PredAIN}   {{\cal PR}_{ain}}
\newcommand{\PredASUB}  {{\cal PR}_{asub}}
\newcommand{\PredL}     {{\cal PR}_{links}}
\newcommand{\PredASUBL} {{\cal PR}_{sublinks}}

%\newcommand{\TRUE}  {{\small \mbox{TRUE}}}

%---------- CHAPTER 6  <OLDVERSION> ---------
%----- S Q L ---------

    \newcommand{\sql}[1]{{\bf #1}}

    \newcommand{\SELVIEW}[1]{
        \sql{SELECTION VIEW} {\em #1}
    }
    \newcommand{\SELVIEWslite}[1]{
        \sql{SELECTION VIEW} #1
    }

    \newcommand{\FROM}[2]{
        \hspace*{1cm} \sql{FROM} {\em #1} \sql{IN} {\em #2}
    }
    \newcommand{\FROMslite}[2]{
        \hspace*{1cm} \sql{FROM} #1 \sql{IN} #2
    }

    \newcommand{\WHERE}[1]{
        \hspace*{1cm} \sql{WHERE} {\em #1}
    }
    \newcommand{\WHEREslite}[1]{
        \hspace*{1cm} \sql{WHERE} #1
    }

%---------------

\newcommand{\oos}[1]{ \mbox{\bf #1} }

%--- UIDS
\newcommand{\printUID}[1]{ \mbox{\em #1} }


\newcommand{\SCuid}[0]      { \printUID{Schema} }

\newcommand{\INuid}[0]      { \printUID{IN} }
\newcommand{\IDuid}[0]      { \printUID{ID} }
\newcommand{\ISAuid}[0]     { \printUID{ISA} }
\newcommand{\NAMEuid}[0]    { \printUID{NAME} }
\newcommand{\ATTRSuid}[0]   { \printUID{ATTR} }
\newcommand{\INSTATTRSuid}[0]{\printUID{INST\_ATTRS} }


%---- Update Sets

\newcommand{\UT}{ UpdateTypes}
\newcommand{\US}{ UpdateState}
\newcommand{\UID}{ UpdateIDs}

\newcommand{\whereT}[0]{
    \mbox{t $\in$ \UT}
}
\newcommand{\Change}{ \mbox{ Changable} }
\newcommand{\Invariant}{ \mbox{ Invariant} }

\newcommand{\Inv}[1]{ \mbox{ Inv[#1]} }
\newcommand{\Ch}[1]{ \mbox{ Ch[#1]} }

\newcommand{\Invv}[2]{ \mbox{ Inv[#1][#2]} }
\newcommand{\Chh}[2]{ \mbox{ Ch[#1][#2]} }

\newcommand{\InvExpl}[1]{ \Invv{Expl}{#1} }
\newcommand{\ChExpl}[1]{ \Chh{Expl}{#1} }

\newcommand{\InvSub}[1]{ \Invv{onSubs}{#1} }
\newcommand{\ChSub}[1]{ \Chh{onSubs}{#1} }

\newcommand{\InvAttr}[1]{ \Invv{onAttrsFrom}{#1} }
\newcommand{\ChAttr}[1]{ \Chh{onAttrsFrom}{#1} }

\newcommand{\InvAttrSub}[1]{ \Invv{onAttrsSubFrom}{#1} }
\newcommand{\ChAttrSub}[1]{ \Chh{onAttrsSubFrom}{#1} }

\newcommand{\Existencial}{\mbox{Existencial}}



\newcommand{\DPATTRNAME}{{\large{{\bf SC}$_{attr}$}}}
\newcommand{\DPISANAME}{{\large{{\bf SC}$_{isA}$}}}
\newcommand{\DPINNAME}{{\large{{\bf SC}$_{in}$}}}

\newtheorem{DP_ATTR}{\DPATTRNAME}
\newtheorem{DP_ISA} {\DPISANAME}
\newtheorem{DP_IN}  {\DPINNAME}


%--- FOR SOURCE CODE

\newcommand{\printKey}[1]{\mbox{\bf #1}}
\newcommand{\mfunction} { \printKey{function} }
\newcommand{\mvar}      { \printKey{var} }
\newcommand{\mset}      { \printKey{SET} }
\newcommand{\mbegin}    { \printKey{begin} }
\newcommand{\mif}       { \printKey{if} }
\newcommand{\melse}     { \printKey{else} }
\newcommand{\mend}      { \printKey{end} }
\newcommand{\mreturn}   { \printKey{return} }

